Unsupervised Summarization Re-ranking

With the rise of task-specific pre-training objectives, abstractive summarization models like PEGASUS offer appealing zero-shot performance on downstream summarization tasks. However, the performance of such unsupervised models still lags significantly behind their supervised counterparts. Similarly to the supervised setup, we notice a very high variance in quality among summary candidates from these models while only one candidate is kept as the summary output. In this paper, we propose to re-rank summary candidates in an unsupervised manner, aiming to close the performance gap between unsupervised and supervised models. Our approach improves the unsupervised PEGASUS by up to 7.27% and ChatGPT by up to 6.86% relative mean ROUGE across four widely-adopted summarization benchmarks ; and achieves relative gains of 7.51% (up to 23.73% from XSum to WikiHow) averaged over 30 zero-shot transfer setups (finetuning on a dataset, evaluating on another).

==> Tables/3_unsup_results.tex <==
\begin{table}[t!]
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
% \textbf{Candidate Selection} 
% & \textbf{Mean R} 
\textbf{Model}
& \textbf{R-1}
& \textbf{R-2}
& \textbf{R-L}
& \textbf{BS}
& \textbf{Gain (\%)} \\

\midrule
\multicolumn{6}{c}{\textit{\textbf{CNN/DM}}} \\
\midrule

% \emph{LEAD-3}                    & \emph{40.05} & \emph{17.48} & \emph{36.35} & \emph{87.19} & \emph{16.01} \\
PEGASUS \cite{zhang2020pegasus}  & 32.90 & 13.28 & 29.38 & \_ & \_ \\
PEGASUS - top beam (ours)        & 35.47 & 13.89 & 31.61 & 86.29 & \_ \\
PEGASUS - random (ours)          & 34.89 & 13.46 & 31.22 & 86.11 & -1.67 \\
\cdashline{1-6}
SummScore - Random-3             & 35.92$^{\dagger}$ & 14.26$^{\dagger}$ & 32.34$^{\dagger}$ & 86.28 & 1.96 \\
\textbf{SummScore - LEAD-3}      & \textbf{36.92}$^{\dagger}$ & \textbf{15.03}$^{\dagger}$ & \textbf{33.19}$^{\dagger}$ & \textbf{86.54}$^{\dagger}$ & \textbf{5.19} \\
SummScore - Salient-R1           & 35.54 & 14.05 & 32.04$^{\dagger}$ & 86.22 & 0.85 \\
SummScore - Salient-R2           & 35.65 & 14.12 & 32.14$^{\dagger}$ & 86.24 & 1.19 \\
SummScore - Salient-RL           & 35.54 & 14.05 & 32.04$^{\dagger}$ & 86.22 & 0.85 \\

\midrule
\multicolumn{6}{c}{\textit{\textbf{XSum}}} \\
\midrule

% \emph{LEAD-3}                    & \emph{19.44} & \emph{2.67} & \emph{12.39} & \emph{86.04} & \emph{0.1} \\
PEGASUS \cite{zhang2020pegasus}  & 19.27 & \textbf{3.00} & 12.72 & \_ & \_ \\
PEGASUS - top beam (ours)        & 18.77 & 2.86 & 13.85 & 85.66 & \_ \\
PEGASUS - random (ours)          & 18.58 & 2.81 & 13.90 & 85.29 & -1.31 \\
\cdashline{1-6}
SummScore - Random-3             & 19.37$^{\dagger}$ & \textbf{2.99}$^{\dagger}$ & 14.52$^{\dagger}$ & 85.78$^{\dagger}$ & 3.89 \\
\textbf{SummScore - LEAD-3}      & \textbf{19.62}$^{\dagger}$ & \textbf{3.02}$^{\dagger}$ & \textbf{14.71}$^{\dagger}$ & \textbf{85.92}$^{\dagger}$ & \textbf{5.24} \\
SummScore - Salient-R1           & 18.96 & 2.88 & 14.19$^{\dagger}$ & 85.65 & 1.52 \\
SummScore - Salient-R2           & 19.13$^{\dagger}$ & \textbf{2.96} & 14.34$^{\dagger}$ & 85.67 & 2.62 \\
SummScore - Salient-RL           & 19.29$^{\dagger}$ & \textbf{2.99}$^{\dagger}$ & 14.48$^{\dagger}$ & 85.79$^{\dagger}$ & 3.63 \\

\midrule
\multicolumn{6}{c}{\textit{\textbf{WikiHow}}} \\
\midrule

% \emph{LEAD-3}                    & \emph{24.38} & \emph{5.54} & \emph{15.64} & \emph{84.89} & \emph{-4.40} \\
PEGASUS \cite{zhang2020pegasus}  & 22.59 & 6.10 & 14.44 & \_ & \_ \\
PEGASUS - top beam (ours)        & 25.49 & 5.91 & 17.99 & \textbf{84.98} & \_ \\
PEGASUS - random (ours)          & 25.39 & 6.00 & 18.09 & 84.82 & -0.38 \\
\cdashline{1-6}
SummScore - Random-3             & 26.29$^{\dagger}$ & \textbf{6.28}$^{\dagger}$ & \textbf{18.78}$^{\dagger}$ & \textbf{84.98} & 3.89 \\
SummScore - LEAD-3               & 26.17$^{\dagger}$ & 6.19$^{\dagger}$ & 18.69$^{\dagger}$ & \textbf{84.96} & 3.16 \\
SummScore - Salient-R1           & \textbf{26.37}$^{\dagger}$ & \textbf{6.32}$^{\dagger}$ & \textbf{18.81}$^{\dagger}$ & \textbf{84.92} & 4.25 \\
\textbf{SummScore - Salient-R2}  & \textbf{26.40}$^{\dagger}$ & \textbf{6.30}$^{\dagger}$ & \textbf{18.83}$^{\dagger}$ & \textbf{84.92} & \textbf{4.37} \\
\textbf{SummScore - Salient-RL}  & \textbf{26.37}$^{\dagger}$ & \textbf{6.32}$^{\dagger}$ & \textbf{18.81}$^{\dagger}$ & \textbf{84.92} & \textbf{4.31} \\

\midrule
\multicolumn{6}{c}{\textit{\textbf{SAMSum}}} \\
\midrule

% \emph{LEAD-3}                    & \emph{30.70} & \emph{8.95} & \emph{23.49} & \emph{86.47} & \emph{17.80} \\
PEGASUS - top beam (ours)        & 26.64 & 6.32 & 22.75 & 86.12 & \_ \\
PEGASUS - random (ours)          & 25.27 & 5.80 & 21.78 & 85.31 & -5.26 \\
\cdashline{1-6}
\textbf{SummScore - Random-3}    & 28.09$^{\dagger}$ & \textbf{7.26}$^{\dagger}$ & \textbf{24.42}$^{\dagger}$ & \textbf{86.39}$^{\dagger}$ & \textbf{7.27} \\
\textbf{SummScore - LEAD-3}      & \textbf{28.22}$^{\dagger}$ & \textbf{7.16} & \textbf{24.39}$^{\dagger}$ & \textbf{86.41}$^{\dagger}$ & \textbf{7.27} \\
SummScore - Salient-R1           & 27.89$^{\dagger}$ & 7.08	& 24.08$^{\dagger}$ & 86.25 & 5.98 \\
SummScore - Salient-R2           & 27.93$^{\dagger}$ & 7.04 & 24.14$^{\dagger}$ & 86.24 & 6.09 \\
SummScore - Salient-RL           & 28.01$^{\dagger}$ & 7.08 & 24.21$^{\dagger}$ & 86.21 & 6.46 \\

\bottomrule
\end{tabular}
}
\caption{\small Unsupervised abstractive summarization results with SummScore re-ranking on the four datasets. PEGASUS is decoded with beam search using 20 beams. \textbf{R-1/2/L} denotes {\sc{Rouge-1/2/L}} and \textbf{BS} denotes BERTScore. \textbf{Gain} represents the mean {\sc{Rouge}} relative gain compared to \emph{our PEGASUS baseline}. $^{\dagger}$ marks indicate significantly better results ($p$-value of paired t-test smaller than 0.05). Best results within 0.1 are in bold.}
\label{tab:3}
\end{table}
